On the bias of K-fold cross validation with stable learners

This paper investigates the efficiency of the K-fold cross-validation (CV) procedure and a debiased version thereof as a means of estimating the generalization risk of a learning algorithm. We work under the general assumption of uniform algorithmic stability. We show that the K-fold risk estimate may not be consistent under such general stability assumptions, by constructing non vanishing lower bounds on the error in realistic contexts such as regularized empirical risk minimisation and stochastic gradient descent. We thus advocate the use of a debiased version of the K-fold and prove an error bound with exponential tail decay regarding this version. Our result is applicable to the large class of uniformly stable algorithms, contrarily to earlier works focusing on specific tasks such as density estimation. We illustrate the relevance of the debiased K-fold CV on a simple model selection problem and demonstrate empirically the usefulness of the promoted approach on real world classification and regression datasets.

==> Preliminaries_back.tex <==
\subsection{Notations}
We place ourselves in the following general learning setting.  One  receives a collection of independent and identically distributed random vectors $\DD=(O_1,\ldots,  O_n)$ 
lying in a sample space $\mathcal Z$, with common distribution $P$. For any $n\in \nset$, let $[n]$ denote the set of integers $\{1,2,\dots,n\}$. Consider a class of predictors $\mathcal{G}$ and a loss function  
%For a predictor $g \in \mathcal G$ and a loss function
$\loss: \mathcal G \times \mathcal Z \to \rset$, so that $\loss(g,O)$
be the error of $g$ on the observation $O\in \mathcal Z$. As an example in
the supervised learning setting
$\mathcal{Z} = \mathcal{X}\times \mathcal{Y}$,  $g$ is a  mapping
$\mathcal{X}\to \mathcal{Y}$ and for $o = (x,y)$ the loss function writes as 
$\ell(g,o) = \ell(g(x), y)$. However our results are not limited to
the supervised setting.  Given a subsample
$\DD_T =\{O_i \mid i \in T \}$ indexed by $T\subset [n]$ and an
algorithm (or learning rule) $\alg$, we denote by
$\alg(T) \in \mathcal G$ the predictor obtained by training $\alg$ on
$\DD_T$. % . In practice, one uses an algorithm $\mathcal{A}$ and a training sample indexed by to pick a suitable model $\alg(\DD_T) \in \mathcal{G}$. Since throughout this paper a single dataset $\DD$ is considered we denote by $\alg(T)$ the predictor $\alg(\DD_T)$. \\
%\begin{remark}
   We consider in this paper deterministic algorithms, that is,  given a subsample $\DD_T$, the output of the algorithm $\alg(T)$ is non random. %In other words, running twice the algorithm on the same subsample produces the same result. %In most examples, this assumption concerns the optimization routine that is employed to run the algorithm.
  We thereby neglect the randomness brought \emph{e.g.} by optimization routines. The case of random algorithms can be covered  at the price of additional notational burden. For the sake of readability we restrict ourselves to  deterministic algorithms  in the main paper and show how to relax it in the supplementary material (Section~\ref{sec:randomized}), in order to cover the case of random algorithms such as Stochastic Gradient Descent (SGD) or neural networks. % .  more technicalities in the proof which we believe would reduce the interpretability of the results.
% % involving the inner-noise level of the algorithm.
%While this includes many standard procedures, it does not take into account the case  when the optimization routine that is used to run the algorithm is not     
%In other words, we don't take into account the \emph{inner} randomness of $\alg$.
\as{ (to be added if we include SGD):  This extension is in particular necessary to one of our counter-examples (Section~\ref{theo:K-fold-LB-SGD}) where we build a lower bound for a SGD algorithm.}
%\end{remark}


The generalization risk of the predictor $\alg(T)$ is 
\[
\TR\big[\alg(T)\big]=\EE\left[ \loss\left(\alg\left(T\right),O\right)\mid \DD_T \right],
\]
where $O$ is independent from $\DD_T$. Notice that the randomness in the latter  expectation stems from  the novel observation $O$ only while the trained algorithm $\alg(T)$ is fixed. %leaving fixed the algorithm $\alg(\DD_T)$.
% Since the distribution $P$ is unknown, so is the generalization risk.
The quantity of interest here is the generalization risk of the learning rule trained on the full dataset, $\TR\big[\alg([n])\big]$. 
The hold-out estimate of the latter involves  a validation index set  $V$ disjoint from $T$ and writes as % (usually $V = [n]\setminus T$)
%is % of the latter consists in 
% one picks a sub sample $V$ and  uses the following risk estimate
\[\ER\big[\alg(T), V\big]=\frac{1}{ n_V} \sum_{i\in V} \loss(\alg(T),O_i),
\]
where %$g \in \mathcal{G}$ and
$n_V=card(V)$. \\
Given a family of validation sets in  $[n]$,  $V_{1:K} = (V_j)_{j=1,\ldots, K}$, 
the \Kfold\xspace\CV  estimator of the generalization risk of $\alg([n])$ is
\begin{equation}\label{def:risk-CV}
\rCV\left[\alg,V_{1 : K}\right]=
\frac{1}{ K} \sum_{j= 1}^{K}\ER\big[\alg({T_j}) , V_j\big],
\end{equation}
where $T_j = [n] \backslash V_j$. % In the sequel we shall often refer to $V_{1:K}$ as the \emph{sequence of masks} because the validation sets are  masked at the training step. 
For clarity reasons, we suppose further that $n$ is divisible by $K$ so that $n/K$ is an integer. This condition guarantees that all validation sets have the same cardinal $n_{V}=n/K$.
% \old{
% \begin{remark}
% While the \Kfold\:procedure is associated to a constant value of $K$ typically ranging between $2$ and $10$ regardless of the sample size $n$, in our generic upper bounds (Theorem~\ref{theo:CV-stable-bound}) we allow the number of folds $K$ to grow with $n$. Allowing this is important in order to include  other popular cross-validation strategyies such as the leave-one-out (\loo)\ where the validation sets $V_i$ are singletons, that is $K=n$. % each validation mask contains one element implying that $K=n$.
% \end{remark}}


\subsection{Algorithmic Stability}
An algorithm $\alg$ is called stable if removing a training point $O_i$ from $\DD_T$ ($i\in T$) or replacing $O_i$ with an independent observation $O'$ drawn from the same distribution does not change much the risk of the output. Formally, for $i\in T \subset [n]$ as above, let $T^{\setminus i }= T\setminus \{i\}$, so that $\alg(T^{\setminus i})$ is the output of $\alg$ trained on $\DD_T\setminus\{O_i\}$. 
Denote similarly  $\alg(T^i)$ the output of $\alg$ trained on $\DD_T\setminus\{O_i\} \cup\{O'\}$. 
%define $\DD_{T^{\setminus i}} $  
%To introduce the stability notion, one needs to construct
% Consider the following modifications of the  dataset~$\DD$, 
% \begin{align*}
% 	\Sot=(O_1,\ldots,O_{l-1},O_{l+1},\dots, O_n)\\
% 	\Scg=(O_1,\ldots,O_{l-1},O',O_{l+1},\dots, O_n).
% \end{align*}
% The dataset $\Sot$ is constructed by omitting the $l$'th element of $\DD$. The sequence $\Scg$ is obtained by replacing the $l$'th element of $\DD$ by $O'$, where $O'$ is an independent observation sampled from the distribution $P$. For the sake of simplicity, we denote  by $\alg(T)$, $\alg^{\backslash l}(T)$, $\alg^l(T)$ the predictors $\alg(\DD_T)$, $\alg(\DD_T^{\backslash l})$ and $\alg(\DD_T^l)$ respectively.

% An algorithm is said to be stable if changing some points in the training set  doesn't affect much his performance. 
The notion of \emph{Hypothesis stability} was first introduced in \cite{DEvroy-79} to derive non asymptotic guarantees for the leave-one-out estimate (\loo). In this paper, we consider instead   \emph{uniform stability}, an assumption used in \cite{bousquet2002stability,wibisono2009,hardt16} to derive probability upper bounds for the training error and the \loo estimate. Equipped with the above notations, \emph{Uniform} stability also called \emph{leave-one-out} stability can be defined as follows.

\begin{definition}\label{def:unif-stable}
	An algorithm $\alg$ is said to be   $(\beta_t)_{1\leq t\leq n}$-\emph{uniformly} stable with respect to a loss function $\loss$ if, for any $T\subset [n]$, $i\in T$ it holds with $P$-probability one that  % $O\in \mathcal{Z}$, it holds that
	\begin{equation}
	\left|\loss\left(\alg(T),O\right)-
	\loss\left(\alg(T^{\backslash i}),O\right)\right| \leq \beta_{n_T}. 
	\end{equation}
      \end{definition}
      % \as{supprimer ce qui suit sur 'change one', et enlever la notation $T^i$? si oui  remplacer par 'notice that slightly weaker notions of stability such as \emph{change-one stability} can be found in the litterature. The latter condition imposes that the  output $\alg(T)$ is close to $\alg(T^i)$,  the output of the algorith trained on $\DD_{T}\setminus\{O_i\}\cup\{O'\}$ where $O'$ is an independent observation sampled from $P$. The formal definition parallels Definition~\ref{def:unif-stable} with $T^i$ in place of  $T^{\setminus i}$    } 
\old{
      If an algorithm is \emph{uniformly} stable, then it is also \emph{change-one} stable.
A related, weaker notion of stability is  \emph{change-one-stability}. The formal definition parallels Definition~\ref{def:unif-stable},  the only difference being, as the name suggests, that $T^{\backslash i}$ is replaced with $T^{i}$.  The link between these two notions is summarized by the following fact.
\begin{fact}\label{fact:uniform-stab-link}
	If an algorithm $\alg$ is  $(\beta_t)_{1\leq t\leq n}$  uniformly stable with respect to a loss function $\loss$ then, $\alg$ is $(2\beta_t)_{1\leq t\leq n}$ \emph{change-one} stable. In other words, for any  $T\subset [n]$, $i\in T$ and $o,o'\in \mathcal{Z}_0\subset  \mathcal{Z}$ where $P(\mathcal{Z}_0) = 1$, the following holds,	
	\[ 
	 \left|\loss\left(\alg(T),o\right)-
	\loss\left(\alg(T^i),o'\right)\right| \leq 2\beta_{n_T}.  
	\]
\end{fact}
We provide the (simple) proof of this result in the appendix for completeness.}
% \begin{proof}
% 	Although the proof of this lemma is simple, we give it in the Appendix for the sake of completeness.
%\end{proof}
\old{
\begin{remark}
	In the literature, \emph{uniform stability} can refer to either  leave-one-out (\cite{bousquet2002stability}) or change-one stability (\cite{hardt16}). In fact,  many popular algorithms (SVM, SGD, Least square regression) verify both hypothesis. However, this breaks up in some special cases, for example, as pointed out in \cite{kutin2002}, if the performance of a learning rule $\alg$  depends on the parity of $n$ then $\alg$ can verify the change one hypothesis without verifying leave-one-out hypothesis.
\end{remark}
.}

% Algorithms $\beta$ uniformly stable are defined such as their fluctuations  when omitting one sample element are less than $\beta$.
% In the next, we claim that when removing $n'$ sample points the fluctuations cannot exceed $n'\beta$.
The following simple fact concerns the effect of removing $n'$ training points on  uniformly stable algorithms. 
\begin{fact}
	\label{fact:Bias-UB}
	Let $\alg$ be a decision rule which is $(\beta_t)_{1\leq t  \leq n}$ uniformly stable, additionally suppose that the sequence $(\beta_t)_{1\leq t  \leq n}$ is decreasing, then for any $T\subset [n]$,  
        % and $O\in \mathcal{Z}$,
        one has, 
	\[\left|\loss\left(\alg\left(\left[n\right]\right),O\right)-
		\loss\big(\alg(T),O\big)\right| \leq \sum_{i=n_T+1}^{n}\beta_i. 
	\]
\end{fact}
\old{Note that the  monotonicity assumption regarding  $(\beta_t)_{1\leq t  \leq n}$ is natural. Indeed, increasing the sample size has an overall stabilizing effect on learning algorithms.} 
\begin{remark}
	Definition \ref{def:unif-stable} and Fact \ref{fact:Bias-UB}  play a key role in our proofs. Namely we use Fact~\ref{fact:Bias-UB} to control the bias of the CV risk estimate and Fact~\ref{def:unif-stable} to derive a probability upper bound on its deviations via McDiarmid's inequality.
\end{remark}

\new{ BALANCE CONDITION REPLACED :
We also need to show that the sequence of training and validation sets of \Kfold\ \CV verifies a certain balance condition.
\begin{fact}\label{fact:mask-property}
	For the \Kfold\ \CV the validation sets $V_1,V_2,\dots V_K$  satisfies
	\begin{equation}\label{"card-condition"}
	card(V_j)=n_V\quad \forall j \in \llbracket1,K\rrbracket,
	\end{equation}
	for some $n_V \in \llbracket1,n\rrbracket$.\,Moreover it holds that %we also assume
	\begin{equation}\label{"key-condition"}
	\frac{1}{K}\sum_{j=1}^{K} {\indic{l \in V_j} }=\frac{n_V}{n} \quad \forall l \in [n]. 
	\end{equation}
\end{fact}
Because $T_j=[n]\backslash V_j$,  if  \eqref{"key-condition"} holds, then the training sets $T_j$ verify a similar equation, that is, 
$$	\frac{1}{K}\sum_{j=1}^{K}  {\indic{l \in T_j} }=\frac{n_{T}}{n} \quad \forall l \in [n].$$
}

% In this paper, our aim is to derive theoretical guarantees for cross validation when the algorithm in our hand is uniformly stable. More formally, we'll make the following assumption.
 % Assumption~\ref{assum:stability-setting} below quantifying the 

Throughout this paper we work under the following uniform stability assumption.
\begin{assumption}[Stable algorithm]
	\label{assum:stability-setting}
	The algorithm $\alg$ is $(\beta_t)_{1\leq t\leq n}$ uniformly stable with respect to a cost function $\loss$ that satisfies,
        $$ %\forall O \in \mathcal{Z} \:,\:
        \forall T \subset [n] ,\:0\leq \loss\left(\alg\left(T\right),O\right) \leq L.$$
	
\end{assumption}

\old{Following the line of \cite{bousquet2002stability} and \cite{hardt16}, we shall consider uniformly stable rules with stability parameter $\beta_n \leq \ffrac{\lambda}{n}$ for some $\lambda>0$.}
\old{ DEPLACE à la fin du theorem 3.1: \begin{discussion*}
	Assumption~\ref{assum:stability-setting}  is indeed verified for many standard  algorithms. In particular $\beta_n=\mathcal{O}(\frac{1}{n})$ for SVM/least square regression with the usual mean squared error, SVM classifier with the soft margin loss (\cite{bousquet2002stability}), SGD  with convex and non convex losses (\cite{hardt16}) and stochastic gradient methods like RGD (randomized coordinate descent), SVRG (stochastic variance reduced gradient method) with loss functions verifying the Polyak-Łojasiewicz condition (\cite{charles18a}). 
\end{discussion*}}


%%% Local Variables:
%%% TeX-master: "main_crossval.tex"
%%% End:


==> detailed-proofs-back.tex <==
\subsection{Proof of Fact \ref{fact:uniform-stab-link}}
The result follow using the following decomposition,
	\begin{align*}
	\abs{\loss\big(\alg(T),O\big)-\loss\big(\alg(T^i,O\big)} &\leq \abs{\loss\big(\alg(T),O\big)-\loss\big(\alg(T^{\backslash i}),O\big)} + \abs{\loss\big(\alg(T^{\backslash i}),O\big)-\loss\big(\alg(T^i),O\big)}\\
	&\leq 2\beta_{\abs{T}},
\end{align*}	
\subsection{Proof of Theorem \ref{theo:CV-stable-bound}}\label{proof:CV-UB}
We proceed as described in the sketch of proof. Using equation \ref{ineq:error-decomp}, write 
\begin{align*}
	\left|\rCV\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right| \leq \abs{\DevCV}+\abs{\BiasCV}.
\end{align*}	
It remains to combine Lemma~\ref{lemma:Dev-CV-UB}, Fact~\ref{fact:Bias-UB}, with the assumption that $\beta_t \leq \ffrac{\lambda}{t}$ to obtain the desired result.
\subsection{Proof of Theorem \ref{theo:K-fold-LB}}\label{sec:proof-LB}
We follow the steps described in the sketch of proof.
To prove the boundedness of $\loss$, notice that for $o = (x,y)\in\mathcal{Z}$, $\DD$ a dataset and $T\subset[n]$, since both $y$ and $\alg(T)(x)$ belong to the interval $[0,\max(\mathcal{X})]$, it holds that 
\begin{align*}
  \ell(\alg[T], o) & = |\alg(T)(x) - y| \le \max(\mathcal{X}) = M S_n. 
\end{align*}

Now since $1/j \le \int_{j-1}^j x^{-1}dx$, %To prove the boundness of $\loss$ it is enough to show that
\begin{align*}
	 S_n = 1 + \sum_{j= 2}^{n}(1/j) &\leq 1 + \int_1^n x^{-1 dx} = \log(n)+1
%	(n \leq \exp(L)) &\leq L^2 +1.
\end{align*}
Since by assumption $\log(n)\le M$ we obtain   $ \ell(\alg[T], o) \le M(\log(n) + 1) \le (M+1)^2$. 
% Indeed, write 
% \begin{align*}
% \log(n)=\int_{1/n}^{1}\frac{dx}{x}&=
% \sum_{j=1}^{n-1}\int_{1/(j+1)}^{1/j}\frac{dx}{x}\\
% & \geq	\sum_{j=1}^{n-1}\frac{1}{j+1}\\
% &= S_n-1,
% \end{align*}
% which concludes the first step.
We now verify that the learning rule defined in \eqref{def:alg-LB} is $3\lambda/n$ uniformly stable. First, notice that under the assumption $0\leq \lambda \leq L(1+\frac{2}{n})^{-1}$ and $0\leq\epsilon\leq \frac{\lambda}{n}$, one has,
$$\alg(T)(x_m)\leq x_m,$$
where $x_m=\sigma_m\varepsilon + LS_m$ is an element of $\mathcal{X}$ (cf. eq \ref{def:X-LB}). Thus, for any $O_m=(x_m,x_m)\in \mathcal{Z}$,
\begin{equation}\label{eq:loss-formula}
	\loss(\alg(T),O_m)=x_m-\alg(T)(x_m).
\end{equation}
Using Equation \ref{eq:loss-formula} and the triangular inequality yields
\begin{align*}
   \abs{\loss(\alg(T),O)- \loss(\alg(T^{\backslash j}),O)}&\leq  \lambda\abs{S_{\min(m,n_{T})}-S_{\min(m,n_{T}-1)}}+2\varepsilon\\
   &=\begin{cases}
   	2\varepsilon + \frac{\lambda}{n_{T}} \quad \text{if} \quad i= n_T\\
   	2\varepsilon 	\quad \text{otherwise}
   \end{cases}\\
(\varepsilon\leq \frac{\lambda}{n_T})  &\leq \frac{3\lambda}{n_T}. 
\end{align*} 
Consequently, $\alg$ is $\ffrac{3\lambda}{n}$ \emph{uniformly} stable. Now, let's compute the true risk of our algorithm, since $P$ is the uniform distribution over $\mathcal{Z}$, we can write, for any $T\subset[n]$,
\begin{align*}
	\risk\left[\alg(T)\right]&=\EE[\alg(T),O \mid \DD_T]\\
	&=\ffrac{1}{n}\sum_{x_m \in \mathcal{Z}}\loss(\alg(T),x_m)\\
(\text{By }\ref{eq:loss-formula})	&=\ffrac{1}{n}\sum_{m=1}^{n}\left(x_m-\alg(T)(x_m)\right)\\
	&=\ffrac{1}{n}\sum_{m=1}^{n}\left(LS_m-\lambda S_{\min(n_T,m)}+ \varepsilon\sign(\med(\DD_T)-x_m)\right).
\end{align*}
Thus, one obtains by simple algebra,
\begin{equation}\label{ineq: bias-LB}
	\ffrac{\lambda}{n}\sum_{m=(n_{T}+1)}^{n}(S_m-S_{n_T})-2\varepsilon  \leq \risk[\alg(T))]- \risk[\alg([n])] 
\end{equation}
To conclude the proof, it remains to derive a lower bound for the left side term in the above equation, to do so write
\begin{align*}
	\ffrac{\lambda}{n}\sum_{m=(n_{T}+1)}^{n}(S_m-S_{n_T})-2\varepsilon &=\ffrac{\lambda}{n}\sum_{m=(n_{T}+1)}^{n}(\sum_{j=(n_{T}+1)}^{m}\frac{1}{j})-2\varepsilon\\
(\frac{1}{j} \geq \frac{1}{n} )	&\geq \ffrac{\lambda}{n^2}\sum_{m=(n_{T}+1)}^{n}(m-n_{T}-1)-2\varepsilon\\
(n_V=n-n_T)&\geq \ffrac{\lambda}{n^2}\sum_{m=1}^{n_V}m-2\varepsilon\\
(\varepsilon \leq \ffrac{\lambda}{n})&\geq \lambda\ffrac{n_V^2}{2n^2} - \ffrac{2\lambda}{n}\\
(n_V=\ffrac{n}{K})&\geq \ffrac{\lambda}{2K^2} - \ffrac{2\lambda}{n}.
\end{align*}
Injecting the above inequality in equation \ref{ineq: bias-LB} gives 
\begin{equation}\label{ineq:bias-Kfold-LB}
\ffrac{\lambda}{2K^2} - \ffrac{2\lambda}{n}	 \leq \risk\left[\alg(T)\right]- \risk\left[\alg([n])\right]. 
\end{equation}
On the other hand, an application of the tower rule yields
\begin{align*}
	\EE\left[\bigg|\rCV\left[\alg,V_{1:K}\right]-\risk\left[\alg([n])\right]\bigg|\right] &= \EE\left[\bigg|\ffrac{1}{K}\left(\sum_{j=1}^{K}\risk\left[\alg(T_j)\right]-\risk\left[\alg([n])\right]\right)\bigg|\right]\\
\big( \risk\left[\alg(T_j)\right]\geq \risk\left[\alg([n])\right]\big)	&=\EE\left[\ffrac{1}{K}(\sum_{j=1}^{K}\risk\left[\alg(T_j)\right]-\risk\left[\alg([n])\right])\right],
\end{align*}
which, using \ref{ineq:bias-Kfold-LB}, gives the desired result.

\subsection{Proof of Theorem \ref{theo:CVC-UB-det}}\label{proof:CVC-UB}
We proceed as described in the sketch of  proof. First remind the error decomposition \ref{ineq:error-decom-cvc}
$$ \rCVC\left[\alg,V_{1:K}\right]-\risk\left[\alg([n])\right] = \DevAll + \ffrac{n_T}{n}(\DevCV+\DevT), $$ 
where $\DevCV$, $\DevT$ and $\DevAll$ are defined in \ref{def:dev_CV}, \ref{def:dev_train} and \ref{def:dev_all} respectively. Since $n_T\leq n$, using the triangular inequality yields
$$ \big|\rCVC\left[\alg,V_{1:K}\right]-\risk\left[\alg[n]\right] \big| \leq \abs{\DevAll} + \abs{\DevCV} +\abs{\DevT} $$
Combining lemma \ref{lemma:Dev-CV-UB} and \ref{lemma:Dev-train-UB} regarding $\DevCV$ and $\DevT$ with Remark \ref{remark:bousquet-UB-gen} regarding $\DevAll$, one obtains, 
\begin{equation}\label{eq:CVC-UB-expon-form}
	\PP\left(\big|\rCVC\left[\alg,V_{1:K}\right]-\risk\left[\alg[n]\right]\big|  -2(\beta_{n_{T}}+\beta_{n}) \geq t\right)\leq 6\exp{\left(\ffrac{-nt^2}{16(\beta_{n_{T}}n_T+L)^2} \right)}.
\end{equation}
By inverting, and using the assumption $\beta_t\leq \ffrac{\lambda}{t}$ one gets, with probability $1-6\delta$,
$$\abs{\rCVC\left[\alg,V_{1:K}\right]-\risk\left[\alg[n]\right]} \leq 2\lambda(\ffrac{1}{n}+\ffrac{1}{n_T}) +4(\lambda+L)\sqrt{\ffrac{\log(1/\delta)}{n}}, $$
which is the desired result.


\subsection{Proof of Theorem \ref{theo:model-selec-CVC}}
The proof of Theorem \ref{theo:model-selec-CVC} relies on the following proposition,
\begin{proposition}\label{prop:uniform-CVC-UB}
	Let $(\alg^{(m)})_{m\in \mathcal{M}}$ be a family of algorithms where each learner $\alg^{(m)}$ is $(\beta_{m,t})_{1\leq i \leq n}$ uniform stable with respect to loss function $0\leq \loss(g,O)\leq L$. Additionally, assume that, $\abs{\mathcal{M}}< \infty$ and,
	$$ \forall m \in \mathcal{M} \:;\: \beta_{m,t} \leq \ffrac{M}{t},$$
	for some $M>0$. Then one has, with probability at least $1-6\delta$,
	\begin{equation*}
		\sup_{m\in \mathcal{M}}\bigg|\ER^{corr}_{\Kfold}\left[\alg^{(m)},V_{1:K}\right]-\TR\big[\alg^{(m)}([n])\big]\bigg|\leq  \ffrac{M(2K-1) }{Kn} +4(M+L)\sqrt{\ffrac{\log(\abs{\mathcal{M}})\log(1/\delta)}{n}}.
	\end{equation*}
\end{proposition}
\begin{proof}
	Using equation \ref{eq:CVC-UB-expon-form} for the \Kfold\:scheme ($n_T=\frac{K-1}{K}$), and the fact that $\beta_{m,n_T} \leq \ffrac{M}{n_T}$. One gets,
	$$ \forall m\in \mathcal{M}\:,\:	\PP\left(\big|\ER^{corr}_{\Kfold}\left[\alg^{(m)},V_{1:K}\right]-\TR\big[\alg^{(m)}([n])\big]\big|  -\ffrac{M(2K-1) }{Kn} \geq t\right)
	\leq 6\exp{\left(\ffrac{-nt^2}{16(\lambda+L)^2} \right)},$$
	which gives by union bound,
	$$ 	\PP\left(\sup_{m\in \mathcal{M}}\big|\ER^{corr}_{\Kfold}\left[\alg^{(m)},V_{1:K}\right]-\TR\big[\alg^{(m)}([n])\big]\big|  -\ffrac{M(2K-1) }{Kn}\geq t\right)
	\leq 6\abs{\mathcal{M}}\exp{\left(\ffrac{-nt^2}{16(\lambda+L)^2} \right)}.$$
	Thus, by inverting, we obtain the desired result.
\end{proof}
\paragraph{Proof of Theorem \ref{theo:model-selec-CVC}} First, using the definition of $\hat m $ (eq \ref{def:opt-Kfold}) write,
$$\ER^{corr}_{\mathrm{Kfold}}\left[ \alg^{(\hat m)},V_{1:K}\right]-\ER^{corr}_{\mathrm{Kfold}}\left[ \alg^{(m^*)},V_{1:K}\right] \leq 0,$$
it follows that,
\begin{align}\label{ineq:key-ineq-mod-selec}
	\risk\big[\alg^{(\hat m)}([n])\big]-\TR\big[\alg^{(m^*)}([n])\big]&\leq   
	\risk\big[\alg^{(\hat m)}([n])\big]-\ER^{corr}_{\mathrm{Kfold}}\left[ \alg^{(\hat m)},V_{1:K}\right]
	+\ER^{corr}_{\mathrm{Kfold}}\left[ \alg^{(m^*)},V_{1:K}\right] -\TR\big[\alg^{(m^*)}([n])\big]\\
	&\leq 2\sup_{m\in \mathcal{M}}\bigg|\ER^{corr}_{\Kfold}\left[\alg^{(m)},V_{1:K}\right]-\TR\big[\alg^{(m)}([n])\big]\bigg|.\nonumber
\end{align}
It remains to use proposition \ref{prop:uniform-CVC-UB} and the proof is complete. 
\section{Uniform stability for randomized algorithms}\label{sec:randomized}
Let's start by reminding the concept of uniform stability for randomized learning algorithms introduced in \cite{elisseeff05a},
\begin{definition}
	An algorithm $\alg$ is said to be   $(\beta_t)_{1\leq t\leq n}$-\emph{uniform} stable with respect to a loss function $\loss$ if, for any $T\subset [n]$, $i\in T$ and $O\in \mathcal{Z}$, the following holds,
	\begin{equation}
	\left|\EE_\alg\left[\loss\left(\alg(T),O\right)-
	\loss\left(\alg(T^{\backslash i}),O\right)\right]\right| \leq \beta_{\abs{T}}. 
	\end{equation}
\end{definition}
Note that a similar version of Facts \ref{fact:uniform-stab-link} and \ref{fact:Bias-UB} still holds, more precisely, one has,
\begin{fact}\label{fact:Bias-UB-randomized}
	If an algorithm $\alg$ is  $(\beta_t)_{1\leq t\leq n}$  uniformly stable with respect to a loss function $\loss$ then, $\alg$ is $(2\beta_t)_{1\leq t\leq n}$ \emph{change-one} stable. In other words, for any  $T\subset [n]$, $i\in T$ and $O,O'\in \mathcal{Z}$, the following holds,	
	\[ 
	\left|\EE_\alg\left[\loss\left(\alg(T),O\right)-
	\loss\left(\alg(T^i),O\right)\right]\right| \leq 2\beta_{\abs{T}}.  
	\]
\end{fact}
\begin{fact}
	Let $\alg$ be a decision rule which is $(\beta_t)_{1\leq t  \leq n}$ uniformly stable, additionally suppose that the sequence $(\beta_t)_{1\leq t  \leq n}$ is decreasing, then for any $T\subset [n]$,  and $O\in \mathcal{Z}$, one has, 
	\[\abs{\EE_\alg\left[\loss\big(\alg([n]),O\big)-
		\loss\big(\alg(T),O\big)\right]} \leq (n-n_{T})\beta_{\abs{T}} . 
	\]
\end{fact}
Now let's derive upper bounds -\emph{in expectation}- on the error induced by $\rCV$ and $\rCVC$.
\begin{theorem}
	Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n\leq \ffrac{\lambda}{n}$, for some $\lambda>0$. Then, we have
	\[ \left|	\EE_{\alg,\DD}\left[\rCV\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right]\right| \leq \ffrac{\lambda n_V}{n_T}. \]
\end{theorem}
\begin{proof}
	First, by applying the tower rule one has,
	\begin{align}\label{eq:CV-expectation-randomized}
		\EE_{\alg,\DD}\left[\rCV\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right]&=\EE_{\alg,\DD}\left[ \frac{1}{ K} \sum_{j= 1}^{K}\ER\big[\alg(T_j) , V_j\big]-\TR\left[\alg([n])\right]\ \right] \nonumber\\
		&=\frac{1}{ K} \sum_{j= 1}^{K}\EE_{\alg,\DD}\left[ \EE_{\alg,\DD}\left[\ER\big[\alg(T_j) , V_j\big]\mid \DD_{T_j}\right]-\TR\big[\alg([n])\big]\ \right] \nonumber\\
		&=\frac{1}{ K} \sum_{j= 1}^{K}\EE_{\alg,\DD}\left[ \EE_{\alg,\DD}\left[\ER\big[\alg(T_j) , V_j\big]\mid \DD_{T_j}\right]-\TR\big[\alg([n])\big]\ \right]\nonumber\\
		&=\frac{1}{ K} \sum_{j= 1}^{K}\EE_{\alg,\DD}\left[ \EE_{\alg,\DD,O}\left[\loss(\alg(T_j,O)-\loss(\alg([n],O))\mid \DD \right] \right].
	\end{align}
	(\ag{je ne sais pas si ici on doit rappeler que pour les algo random le risque s'écrit comme $\risk(\alg(T)=\EE_{\alg,O}[l(\alg(\DD_T),O)]$ parce qu'on peut aussi laisser la définition $\TR\big[\alg(T)\big]=\EE\left[ \loss\left(\alg(T),O\right)\mid \DD_T \right]$  et l'espérance incluera aussi la "randomness" de $\alg$})		
	The last line follows from the fact that, if $O$ is independent from $\DD$ then for all $j \in V$ , $\loss(\alg(T),O_j)$ and $\loss(\alg(T),O)$ has the same law . \\
	To obtain the desired result, it remains to combine Equation \ref{eq:CV-expectation-randomized} with fact \ref{fact:Bias-UB-randomized}.
\end{proof}
The latter Theorem will serve as a tool to prove the \emph{l-p-o}  consistency.
\begin{corollary}
	[\emph{l-p-o} consistency]
	Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n\leq \ffrac{\lambda}{n}$, for some $\lambda>0$. Then, we have,
	\[ \left|	\EE_{\alg,\DD}\left[\ER_{\mathrm{lpo}}\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right]\right| \leq \ffrac{\lambda p}{n-p}. \]
\end{corollary}
Now let's prove that the bias corrected \Kfold\:(cf. Eq \ref{def:risk-CV-corr}) is indeed consistent for randomized algorithms.
\begin{theorem}[Corrected \Kfold\;consistency]
	Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n\leq \ffrac{\lambda}{n}$, for some $\lambda>0$. Then, we have,
	\[ \left|	\EE_{\alg,\DD}\left[\ER_{\mathrm{Kfold}}^{corr}\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right]\right| \leq \ffrac{2\lambda(2K-1)}{Kn}. \]
\end{theorem}
\begin{proof}
	Combining the error decomposition \ref{ineq:error-decom-cvc} with the fact that  $n_T=\ffrac{K-1}{K}n$ we obtain :
	\begin{equation}\label{eq:CVC-decomp-Kfold}
	\ER_{\mathrm{Kfold}}^{corr}\left[\alg,V_{1:K}\right]-\risk\left[\alg[n]\right] = \DevAll+ \ffrac{K-1}{K}(\DevCV+\DevT).
	\end{equation}
	
	Using  Theorem 2.2 in \cite{hardt16}, one obtains, the twin inequality,
	\[ \left|\EE_{\alg,\DD}\left[\DevAll\right]\right| \leq 2\beta_n \]
	\[ \left|\EE_{\alg,\DD}\left[\DevT\right]\right| \leq 2\beta_{n_T}.  \]	
	Since $\EE_{\alg,\DD}\left[\DevCV\right]=0$, Equation \ref{eq:CVC-decomp-Kfold} combined with the triangular inequality gives,
	\begin{align}\label{ineq:random-Kfold}
		\left|	\EE_{\alg,\DD}\left[\ER_{\mathrm{Kfold}}^{corr}\left[\alg,V_{1:K}\right]-\TR\big[\alg([n])\big]\right]\right| &\leq 2\left(\beta_n+\ffrac{(K-1)\beta_{n_T}}{K}\right) \nonumber\\
		&\leq 2\left(\beta_n+\beta_{n_T}\right).
	\end{align}
	It remains to use the assumption $\beta_t\leq \ffrac{\lambda}{t}$ and the proof is complete.	
\end{proof}
We conclude this section by deriving an upper bound for the model selection problem,
\begin{theorem}	Let $(\alg^{(m)})_{m\in \mathcal{M}}$ be a family of algorithms where each learner $\alg^{(m)}$ is $(\beta_{m,t})_{1\leq i \leq n}$ uniform stable with respect to loss function $0\leq \loss(g,O)\leq L$. Additionally, assume that, 
	$$ \beta_{m,t} \leq \ffrac{M}{t},$$
	for some $M>0$, then one has,
	\[\EE_{\alg,\DD}\left[\risk\big[\alg^{(\hat m)}([n])\big]-\TR\big[\alg^{(m^*)}([n])\big]\right] \leq \ffrac{4M(2K-1)}{Kn}.\]
	where $m^*$ and $\hat m $ are defined by Equations \ref{def:oracle}, \ref{def:opt-Kfold} respectively.
\end{theorem}
\begin{proof}
	First, using Equation \ref{ineq:random-Kfold}, one obtains, for all $m\in \mathcal{M}$,
	\begin{align*}
		\left|\EE_{\alg,\DD}\left[\ER_{\mathrm{Kfold}}^{corr}\big[\alg^{(m)},V_{1:K}\big]-\TR\big[\alg^{(m)}([n])\big]\right]\right| &\leq 2\left(\beta_{m,n}+\beta_{m,n_T}\right)\\
		&\leq \ffrac{2M(2K-1)}{Kn}.
	\end{align*}
	So that
	\begin{equation}\label{ineq:exp-model-selec-UB}
	\sup_{m\in\mathcal{M}}\left|\EE_{\alg,\DD}\left[\ER_{\mathrm{Kfold}}^{corr}\left[\alg^{(m)},V_{1:K}\right]-\TR\big[\alg^{(m)}([n])\big]\right]\right|\leq \ffrac{2M(2K-1)}{Kn}. 
	\end{equation}
	On the other hand, Inequality \ref{ineq:key-ineq-mod-selec} yields,
	\begin{align*}
		\EE_{\alg,\DD}\left[\risk\big[\alg^{(\hat m)}([n])\big]-\TR\big[\alg^{(m^*)}([n])\big] \right]&\leq  
		\EE_{\alg,\DD}\left[\risk\big[\algdd^{(\hat m)}([n])\big]-\ER^{corr}_{\mathrm{Kfold}}\big[ \alg^{(\hat m)},V_{1:K}\big]\right]\\&\hspace{8mm}
		+\EE_{\alg,\DD}\left[\ER^{corr}_{\mathrm{Kfold}}\big[ \alg^{(m^*)},V_{1:K}\big] -\TR\big[\alg^{(m^*)}([n])\big]\right]\\
		&\leq 2\sup_{m\in\mathcal{M}}\left|\EE_{\alg,\DD}\left[\ER_{\mathrm{Kfold}}^{corr}\big[\alg^{(m)},V_{1:K}\big]-\TR\big[\alg^{(m)}([n])\big]\right]\right|.
	\end{align*}
	Thus, by Inequality \ref{ineq:exp-model-selec-UB}, one has,
	$$	\EE_{\alg,\DD}\left[\risk\big[\alg^{(\hat m)}([n])\big]-\TR\big[\alg^{(m^*)}([n])\big] \right] \leq \ffrac{4M(2K-1)}{Kn},$$
	which concludes the proof.
\end{proof}

\ag{remarque: noter $n_T$ ou $\abs{T}$ dans tout le papier}
%%% Local Variables:
%%% TeX-master: "main_crossval.tex"
%%% End:


==> deterministic-alg.tex <==
Our first main result Theorem~\ref{theo:CV-stable-bound} below holds true for any \CV procedure verifying assumption \ref{assum:mask-property}.
\begin{theorem}\label{theo:CV-stable-bound}
 Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n=\ffrac{\lambda}{n}$, for some $\lambda>0$. Then, for all CV schemes verifying Assumption \ref{assum:mask-property},  we have, with probability $1-2\delta$,
 \begin{align*}
 	\bigg|\rCV(\alg,V_{1:K})-\TR\big[&\algdd([n])\big]\bigg|\leq \lambda\frac{n_V}{n}\\&+4(\lambda+L)\sqrt{\ffrac{\log(1/\delta)}{n}}.
 \end{align*}

Where $L$ is the upper bound of the cost function $\loss$.	
\end{theorem}

\begin{proof}[sketch of proof]
	Define the average risk of the family $\big(\alg(\DD_{T_j})\big)_{1\leq j \leq K}$
	\begin{equation}\label{eq:true-rcv-def}
		\risk_{CV}(\alg,V_{1:K})= \frac{1}{K}\sum_{j=1}^{K}\risk\big[\algdd(T_j)\big],
	\end{equation}
	then write the following decomposition 
	\begin{equation}\label{ineq:error-decomp}
		\rCV(\alg,V_{1:K})-\TR\big[\algdd([n])\big] = \DevCV+\BiasCV,
	\end{equation}
	with \begin{align}
	&\DevCV= \rCV(\alg,V_{1:K})-  \risk_{CV}(\alg,V_{1:K})\label{def:dev_CV},  \\
	&\BiasCV= \mathcal{R}_{CV}(\alg,V_{1:K})-\TR\big[\algdd([n])\big]\label{def:bias_CV}. 
	\end{align}
	The proof consists in bounding each term of the above decomposition independently. The term $\DevCV$ measure the deviations of $\rCV$ from it's mean and it can be controlled using Mcdiarmid's inequality (Proposition \ref{prop:Mcdiarmids-ineq}). For the second term, the control is provided by Corollary \ref{lemma:uniform-stab-link}. The detailed proof is deferred to the appendix.
\end{proof}
\begin{discussion*}
	Applying Theorem \ref{theo:CV-stable-bound} to the leave-one-out procedure ($n_V=1$) gives the same bound as in Theorem 12 (\cite{bousquet2002stability}). Thus, it turns out that, our result can be seen as an extension of the previous work to a wider class of $\CV$ schemes.
\end{discussion*}
In the rest of this section, we will apply Theorem \ref{theo:CV-stable-bound} to control the  estimation error of some usual \CV procedures, in particular \emph{leave-$p$-out} and \Kfold \: \CV. 
\begin{corollary}[\emph{l-p-o} upper bound]
	Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n=\ffrac{\lambda}{n}$, for some $\lambda>0$. Then, we have, with probability $1-2\delta$,
	\begin{align*}
		\bigg|\ER_{\mathrm{lpo}}(\alg,V_{1:K})-\TR\big[\algdd(&[n])\big]\bigg|\leq \frac{\lambda p}{n}\\&+4(\lambda+L)\sqrt{\frac{\log(1/\delta)}{n}}.
	\end{align*}
	Where $\ER_{\mathrm{lpo}}$ is the \emph{l-p-o} estimate, and $L$ is the upper bound of the cost function.	
\end{corollary}
\begin{proof} By Lemma \ref{lemma:CV-scheme-property} we know that  \emph{l-p-o} CV verifies assumption \ref{assum:mask-property}, thus  applying Theorem \ref{theo:CV-stable-bound} with $n_V=p$ yields the desired result . 	
\end{proof}
Similar arguments can be applied to show the following corollary regarding \Kfold  scheme.
\begin{corollary}[$K$-fold upper bound]
	 Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n=\ffrac{\lambda}{n}$, for some $\lambda>0$. Then, we have, with probability $1-\delta$,
	 \begin{align*}
	 \bigg|\ER_{\mathrm{Kfold}}(\alg,V_{1:K})-\TR\big[\algdd(&[n])\big]\bigg|\leq \frac{\lambda}{K}\\&+4(\lambda+L)\sqrt{\frac{\log(1/\delta)}{n}}.
	 \end{align*}
	 Where $\ER_{\mathrm{Kfold}}$ is the $K$-fold estimate, and $L$ is the upper bound of the cost function.	
\end{corollary}
\begin{remark}
	In the above corollary, the upper bound isn't consistent in the sense that, it doesn't tend to $0$ as $n \rightarrow \infty$. A natural question arises, can we derive consistent probability bound for \Kfold\:procedure? \\
	In the next section, we show that the answer to this question is rather negative.
\end{remark}
\subsection{Lower bound for \Kfold\:\CV}
The next result highlights the following fact, under uniform stability assumption alone, one cannot obtain any  theorical guarentees about the consistency of \Kfold\:\CV. 
\begin{theorem}[$K$-fold inconsistency]\label{theo:K-fold-LB} Let $0\leq \lambda \leq L(1+\ffrac{2}{n})^{-1}$ and an integer $n\ \leq \floor{\exp{(L)}}$ . There exists an algorithm $\alg$ verifying assumption \ref{assum:stability-setting} with $\beta_n=\lambda/n$, a sample space $\mathcal{Z}$, a distribution $P$ such as,
	$$\EE\left[\big|\ER_{\mathrm{Kfold}}\left(\alg,V_{1:K}\right) - \risk\left[\alg([n])\right]\big| \right] \geq \frac{\lambda}{K^2}-\ffrac{2\lambda}{n}.$$
	
\end{theorem}

\begin{proof}[sketch of proof]
	The idea of this proof is inspired from \cite{liu2021tight}. First, we create a discrete space of size $n$,
	\begin{equation}\label{def:X-LB}
		\mathcal{X}=\left\{\sigma_1\varepsilon+LS_1,\sigma_2\epsilon+LS_2,\dots,\sigma_n\varepsilon+LS_n\right\},
	\end{equation}
	where $0<\varepsilon<\ffrac{\lambda}{n}$, $\sigma_m=\indic{m \leq \floor{n/2}}-\indic{m > \floor{n/2}}$ and $S_m=\sum_{j=1}^{m}(1/j)$. Then, by using $\mathcal{X}$, construct the sample space as follow $\mathcal{Z}=\left\{(x,x)\mid x\in \mathcal{X} \right\}$, in other words, we consider a regression problem where $X=Y$.\\
	Now, let's draw a sample $$D=\{(x_1,y_1),(x_2,y_2),\dots,(x_n,y_n)\}$$ from $\mathcal{Z}$ using a uniform distribution $P$. For a training sequence indexed by $T\subset [n]$, for a given $x_m=\sigma_m\varepsilon+LS_m \in \mathcal{X}$, define the learning rule,
	\begin{equation}\label{def:alg-LB}
			\algdd(T,x_m)=\lambda S_{\min(m,n_T)}+\varepsilon\sign(\med(\DD_T)-x_m).
	\end{equation}

	
	The intuition behind our algorithm is the following, the term $\sign(\med(\DD_T)-x_m)$ tries to capture the sign of $\epsilon$ and the term $\lambda S_{\min(m,n_T)}$ controls the \emph{intensity} of the output. Clearly, our rule is way better than a random guess.\\
	
	For an observation $O=(x,y)$, take as a loss function $l(\algdd(T) , O)=\abs{\algdd(T,x) -y}$ and proceed following this steps,
	\begin{enumerate}
		\item Show that $\loss$ is $L^2$-bounded.
		\item Verify the uniform stability assumption i.e, for any training mask $T \subset [n]$, index $j\in T$ and observation $O\in \mathcal{Z}$, one has,
		$$ \abs{\loss(\algdd(T),O)- \loss(\algdd(T^{\backslash j}),O)}\leq \frac{\lambda}{n_T}.$$
		\item Compute the true risks $\risk\left(\algdd(T)\right)$ and $\risk\left(\algdd([n])\right)$.
		\item Deduce that $\risk\left(\algdd(T)\right)- \risk\left(\algdd([n])\right) \geq \ffrac{\lambda}{K^2}-\ffrac{2\lambda}{n}.$
	\end{enumerate}
	
	After this steps, an application of the tower rule yields the desired result. The technical details are gathered in Appendix \ref{sec:proof-LB}.	
\end{proof}
\begin{discussion*}
	This theorem reflects the known suboptimality of \Kfold\:CV. Indeed, It was shown in several contexts that performing \Kfold\:can be misleading. For example, in a linear regression framework, \cite{Yuhong2007} has shown that the usual 5-fold procedure cannot select the right model.
\end{discussion*}

We can conclude from this section, that only \emph{l-p-o} CV schemes are consistent. However in practice, this kind of procedures is computationally heavy since we need to train our model at least $n$ times. In the next section, we will show that adding the correction terms (\cite{BURMAN89}) to $K$-fold \CV improves the quality of this procedure drastically.
\section{Elegant cross validation}
The bias corrected cross validation $\rCVC$ was shown to be more accurate than the standard  CV procedures in certain cases. To be more precise, adding the correction terms can delete the bias of cross validation when the algorithm in hand verifies some smoothness assumptions. Here, we show that, this method  outperforms the usual CV schemes even in a more general framework : the framework of stable learners.
\begin{theorem}
\label{theo:CVC-UB-det}
 Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n=\ffrac{\lambda}{n}$, for some $\lambda>0$. Then, for all CV schemes verifying Assumption \ref{assum:mask-property},  we have, with probability $1-6\delta$,
 \begin{align*}
 	\bigg|\rCVC(\alg,V_{1:K})-\TR\big[&\algdd([n])\big]\bigg|\leq  2\lambda(\ffrac{1}{n}+\ffrac{1}{n_T})\\ &+4\ffrac{n_T(\lambda+L)}{n}\sqrt{\ffrac{\log(1/\delta)}{n}}.
 \end{align*}

\end{theorem}

\begin{proof}[sketch of proof]
	
	By simple algebra write 
	\begin{align*}
	\rCVC(\alg,&V_{1:K}) = \ER\left(\algdd([n]),[n]\right) \\+ &\ffrac{n_T}{nK}\sum_{j=1}^{K}\left[\ER(\alg(T_j),V_j)-\ER(\alg(T_j),T_j)\right] .
	\end{align*}
	Using the previous equation, deduce the following decomposition
	\begin{equation}
	\rCVC(\alg,V_{1:K})-\risk(\alg[n]) = \DevAll+ \ffrac{n_T}{n}(\DevCV+\DevT).\label{ineq:error-decom-cvc}
	\end{equation}
	Where $\DevCV$ is  defined in \ref{def:dev_CV} and 
	\begin{align}
	\DevAll &= \ER(\alg[n],[n])-\risk(\alg[n])\label{def:dev_all}\\
	\DevT &=\ffrac{1}{K}\sum_{j=1}^{K} \left(\risk\big[\alg(T_j)\big]-\ER(\alg(T_j),T_j)\right).\label{def:dev_train}
	\end{align}
	The remaining part of the proof consist in bounding each term of the previous decomposition independently. To be more precise, we use Mcdiarmid's inequality (proposition \ref{prop:Mcdiarmids-ineq}) to bound both $\DevCV$ and $\DevT$. Then, we derive a probability upper bound for $\DevAll$ directly from  proposition \ref{prop:ER-stability-bound}. The detailed proof is deferred to the appendix
\end{proof}
Theorem \ref{theo:CVC-UB-det} allows to obtain a consitent bound for \Kfold\:\CV.
\begin{corollary}
	Suppose that Assumption~\ref{assum:stability-setting} holds with $\beta_n=\ffrac{\lambda}{n}$, for some $\lambda>0$. Then, for corrected \Kfold\:\CV,  we have, with probability $1-6\delta$,
	\begin{align*}
		\bigg|\ER^{corr}_{\Kfold}(\alg,V_{1:K})-\TR\big[&\algdd([n])\big]\bigg|\leq  \ffrac{\lambda(2K-1) }{Kn}\\ &+4\ffrac{(K-1)(\lambda+L)}{K}\sqrt{\ffrac{\log(1/\delta)}{n}}.
	\end{align*}
\end{corollary}
\begin{proof}
	Remind that $n_T=\frac{K-1}{K}n$ for the \Kfold\:scheme. Thus, applying Theorem \ref{theo:CVC-UB-det} gives the desired result.
\end{proof}
The former corollary  confirms the consistency in estimation of the bias corrected \Kfold\:for \emph{uniformly} stable learners. However, in practice, one uses cross validation for model selection, which can be far away from risk estimation. In the next section, we show that, the bias corrected cross validation is also consistent in model selection when using uniformly stable algorithms.



==> experiments.tex <==
The aim of our experiments is to illustrate empirically the added
value of the corrected \Kfold\ compared with the standard one in
terms of efficiency in model selection. In other words we perform
model selection with the \Kfold\ and the corrected version that we
promote and we compare the generalization risks  of the selected
trained models.

\subsection{Experimental Setting}

% In this section, we will compare the performances of a model selected by the usual \Kfold\:CV with the performance a model selected by the bias corrected \Kfold.
We choose as a family of models $\mathcal{M}$  a family of  SVM regressors and classifiers trained with a regularization parameter $\gamma_m$ ranging in a finite grid in an interval $[a,b]$.
Namely we set $[a,b]=[0.1,100]$, and the grid is constructed with a  constant step size equal to $\Delta = 0.1$, so that $$(\gamma_m)_{m\in \mathcal{M} }=\{a+j\Delta \mid 0 \leq j < 1000\}.$$ 
 In this SVM framework, 
$$\alg^{(m)}(T)=\argmin_{f\in \mathcal{F}}\ffrac{1}{n_T} \sum_{i\in T}\loss(f,O_i)+\gamma_m \lVert f \rVert_k$$
where $\mathcal{F}$ is  a reproducing kernel Hilbert space with kernel $k$. We use the implementation provided by the python library \texttt{scikit-learn}. The kernel $k$ is chosen here as the sigmoid kernel $\tanh( \tau \langle x, \rangle )$ . Following standard practice we set  $\tau=\frac{1}{d}$, where $d$ is the dimension of the dataset. % variances. 
%One wants to pick the best model $m^*$ defined by \ref{def:oracle}.
%We will suppose that one searches the best regularization parameter in a grid $[a,b]$ so that we can stay in the settings of
The assumptions of Theorem~\ref{theo:model-selec-CVC} are thus satisfied, as pointed out in the discussion following the theorem's statement.
We  use the quadratic loss for regression problems and  the hinge loss $\loss(g,(x,y))= (1-yg(x))_{+}$ for classification, where $(f(x))_+=max(0,f(x))$.  Since the training datasets are bounded, we may consider that  both these losses as bounded as well. For both these losses the algorithm $\alg^{(m)}$ is $\ffrac{\lambda}{n}$ uniformly stable (see \cite{bousquet2002stability} for further details).
\subsection{Datasets} %Comparison between the bias corrected \Kfold\: and the usual \Kfold}
Eight reference datasets from UCI \footnote{\url{https://archive.ics.uci.edu}} are considered: four classification datasets and four regression datasets listed below.
\paragraph{Regression datasets } \emph{Real estate valuation} (REV, 414 house price of unit area with 5 covariates); \emph{QSAR fish toxicity } (906 toxic chemical concentration with 6 attributes); \emph{Energy efficiency} (EE, 768 heating loads with 8 features.); \emph{Concrete Compressive Strength} (CS, 1030 measure of the compressive strength with 8 attributes).
\paragraph{Classification datasets }\emph{Ionosphere dataset} (IO, 351 radar returns with 34 attributes), \emph{Raisin dataset} (RS, 900 Keciman/Besni raisin with 7 attributes), \emph{Audit risk dataset} (AR, 777 firm evaluation (fraudulent/non fraudulent) with 18 risk factors) and \emph{QSAR bio degradation Data Set } (BIODEG, 1055 chemicals categorization with 12 descriptive features). 


For  each dataset one third of the data  are removed ($\mathcal{S}$)  and reserved for testing, \ie for evaluating the generalization risk of the  model selected using the remaining two thirds ($\DD$). 
%re we  take one third for testing ($\mathcal{S}$) and two thirds for training ($\DD$)
Let  $\hat m_{\mathrm{Kf}}$ (\emph{resp.} $\hat m_{\mathrm{Kf-corr}}$)  denote the model selected using \Kfold \ \CV\ (\emph{resp.} corrected \Kfold\ \CV)   on the train set $\DD$. In other words
\begin{equation*}
\begin{aligned}
		 \alg^{(\widehat m_{\mathrm{Kf-corr}})}&=\argmin_{m\in \mathcal{M}}\ER^{corr}_{\mathrm{Kfold}}\left[ \alg^{(m)},V_{1:K}\right], \\
		 \alg^{(\widehat{m}_{\mathrm{Kf}})}&=\argmin_{m\in \mathcal{M}}\ER_{\mathrm{Kfold}}\left[ \alg^{(m)},V_{1:K}\right].
\end{aligned}
\end{equation*}
In the end, in line with Section~\ref{sec:model-selec}, the performance of both models are compared in terms of generalization risk using the empirical risk on the test set $\mathcal{S}$,
\begin{equation}
  \label{eq:gene-risk-test}
  \ER\left[\alg_{\DD}^{(\hat m)},\mathcal{S}\right]=\ffrac{1}{n_{\mathcal{S}}}\sum_{O_i \in \mathcal{S}}l\left(\alg^{(\hat m)}([n]),O_i\right) .
\end{equation}
\subsection{Results}
Tables~\ref{table:regression-results} and~\ref{table:classification-results} gather the results obtained respectively with the regression and classification datasets, for different numbers of folds $K$ variying between $2$ and $5$.   In all  cases, the model selected by the bias corrected \Kfold\: has a lower generalization risk than the one selected by the standard \Kfold.  As expected,  the standard  \Kfold\:procedure behaves generally  better with  $K=5$ than with $K=2$. Indeed larger values of $K$ decrease the bias of the \Kfold\ \CV. The benefit of the bias correction is thus all the more important for small values of $K$. 
\begin{table}[!h]
	\caption{Regression mean squared errors for the \Kfold\: and the bias corrected \Kfold\:
		on various data sets.}
	\label{table:regression-results}
	\vskip 0.15in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lcccr}
					\hline
					Dataset & K-fold & Bias corrected K-fold \\ 
					\hline
      			REV; K=3 & 74.198 & \textbf{68.958} \\ 
					REV; K=4 & 74.189 & \textbf{68.958} \\ 
					REV; K=5 & 73.359 & \textbf{68.958} \\ 
					\hline
					EE; K=3 & 15.501 & \textbf{14.405} \\ 
					EE; K=4 & 15.825 & \textbf{14.35} \\ 
					EE; K=5 & 14.73 & \textbf{14.298} \\ 
					\hline
					QSAR; K=3 & 1.183 & \textbf{1.035} \\ 
					QSAR; K=4 & 1.112 & \textbf{1.035} \\ 
					QSAR; K=5 & 1.112 & \textbf{1.035} \\ 
					\hline
					CS; K=3 & 146.881 & \textbf{126.492} \\ 
					CS; K=4 & 144.195 & \textbf{124.205} \\ 
					CS; K=5 & 137.06 & \textbf{123.641} \\ 
				%	\hline
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	\vskip -0.1in
    \end{table}
\begin{table}[!h]
	\caption{Hinge losses for the \Kfold\: and the bias corrected \Kfold\:
		on various data sets.}
	\label{table:classification-results}
	\vskip 0.15in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lcccr}
					\hline
					Dataset & K-fold & Bias corrected K-fold \\ 
					\hline
					RS; K=3 & 0.47 & \textbf{0.419} \\ 
					RS; K=4 & 0.42 & \textbf{0.418} \\ 
					RS; K=5 & 0.42 & \textbf{0.419} \\ 
					\hline
					IO; K=3 & 0.454 & \textbf{0.414} \\ 
					IO; K=4 & 0.447 & \textbf{0.425} \\ 
					IO; K=5 & 0.477 & \textbf{0.464} \\ 
					\hline
					BIODEG; K=3 & 0.361 & \textbf{0.357} \\ 
					BIODEG; K=4 & 0.363 & \textbf{0.357} \\ 
					BIODEG; K=5 & 0.381 & \textbf{0.357} \\ 
					\hline
					AR; K=3 & 0.112 & \textbf{0.109} \\ 
					AR; K=4 & 0.108 & \textbf{0.105} \\ 
					AR; K=5 & 0.107 &  \textbf{0.106} \\ 
					\hline
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	\vskip -0.1in
\end{table}


%%% Local Variables:
%%% TeX-master: "main_crossval.tex"
%%% End:

      

==> intermediate-old.tex <==


First we bound -in probability- $\DevCV$  defined by  \eqref{def:dev_CV}.


\begin{lemma}\label{lemma:Dev-CV-UB}
 Suppose that Assumption~\ref{assum:stability-setting} holds. Then, for all CV schemes verifying Assumption \ref{assum:mask-property},  we have
	\begin{equation*}
	\PP(\abs{\DevCV} \geq t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}.
	\end{equation*}

\end{lemma}
\begin{proof} 
	Let  $O'\in \mathcal{X}$ be  an independent copy of $O_1,O_2,\dots,O_n$, for any $l\in \llbracket1,n\rrbracket$ define 
	\[\Delta_l(\DD,O')=\big\lvert \DevCV(\DD)-\DevCV(\DD^l)\big\rvert, \]
	where $\DD^{l}$ is obtained by replacing the $l$'th element of $\DD$ by $O'$. Now we derive an upper bound on $\PP(\abs{\DevCV} \geq t)$ using Proposition \ref{prop:Mcdiarmids-ineq}. Namely, we will bound the maximum deviation of $\Delta_l$ by $\Delta_l \leq  \ffrac{4\beta_{n_{T}} n_{T}}{n}+\ffrac{L}{n}$. To do so, write 
	\begin{align*}
	\DevCV&=\rCV\left[\alg,V_{1:K}\right]-  \risk_{CV}\left[\alg,V_{1:K}\right]\\
	&=\frac{1}{Kn_{val}}\sum_{j=1}^K\sum_{i \in V_j} \bigg(\loss(\alg (T_j),O_i)-\EE_{O}\big[\loss(\alg(T_j),O) \mid \DD_{T_j})\big]\bigg)\\
	&=\frac{1}{Kn_{val}}\sum_{j=1}^K\sum_{i \in V_j}h(\alg(T_j),O_i),
	\end{align*}
	where the last is used to define $h$. For a training mask $T_j\subset [n]$, let $\alg(T_{j,l}) $ denote the algorithm $\alg$ trained on the sequence $\DD_{T_j,l}=\{O_i \in \DD^{l} \mid i \in T_j\}$. Note that, for all $ \DD_{T_j},o \in \mathcal{Z}^{n_{T}}\times \mathcal{Z}$ one has 
	\begin{equation}
	\label{"train_set_dev"}
	\begin{cases}
	\loss\big(\alg(T_j),o\big)=\loss\big(\alg(T_{j,l}),o\big)\: \text{if} \: l \notin T_j\\
	\bigg \lvert \loss\big(\alg(T_j),o\big)-\loss\big(\alg(T_{j,l}),o\big) \bigg\rvert \leq 2\beta_{n_{T}}\:,\: \text{otherwise}.
	\end{cases}
	\end{equation}
	The first equation follows from the fact that $\DD_{T_j,l}=\DD_{T_j}$ if $l\notin T_j$, indeed, if the training set $\DD_{T_j}$ doesn't contain the index $l$ then changing the $l$'th element of $\DD$ won't affect $\DD_{T_j}$.\,The second inequality is obtained using the \emph{uniform} stability of $\alg$ and fact \ref{fact:uniform-stab-link}. Furthermore, using Equation \ref{"train_set_dev"} write
	\begin{equation}
	\label{"expectation_train_set_dev"}
	\begin{cases}
	\EE\bigg[\loss\big(\alg(T_j),O\big)\mid \DD_{T_{j}}\bigg]=\EE\bigg[\loss\big(\alg(T_{j,l}),O\big)\mid \DD_{T_{j,l}}\bigg]\: \text{if} \: l \notin T_j\\
	\bigg \lvert \EE\big[\loss\big(\alg(T_j),O\big)\mid \DD_{T_j}\big]- \EE\big[\loss\big(\alg(T_{j,l}),O\big)\mid \DD_{T_{j,l}}\big] \bigg\rvert \leq 2\beta_{n_{T}} , \: \text{otherwise}.
	\end{cases}
	\end{equation}
	
	Combining \eqref{"expectation_train_set_dev"} and \eqref{"train_set_dev"} gives
	\begin{equation}
	\label{eq:key-DCV-Mcdiarmid}
	\begin{cases}
	\abs{\un{l \in T_j}(h(\alg(T_j),O_i))-h(\alg(T_{j,l}),O_i))} \leq 4\beta_{n_{T}}\\
	\abs{\un{l \notin T_j}(h(\alg(T_j),O_i))-h(\alg(T_{j,l}),O_i)) }\leq L\un{i=l}.	
	\end{cases}
	\end{equation}
	So that
	\begin{align*}
	\abs{\Delta_l(\DD,O')}&\leq  \frac{1}{Kn_{val}}\sum_{j=1}^K\sum_{i \in V_j}\abs{h(\alg(T_j),O_i))-h(\alg(T_{j,l}),O_i))} \\
	(T_j^c=V_j)&=\frac{1}{Kn_{val}}\sum_{j=1}^K\sum_{i \in V_j}\abs{h(\alg(T_j),O_i))-h(\alg(T_{j,l}),O_i))}\left(\un{l\in T_j}+\un{l\in V_j}\right)\\
	(\text{By Equation \ref{eq:key-DCV-Mcdiarmid}} ) &\leq \ffrac{4\beta_{n_{T}}}{K}\sum_{j=1}^{K}\un{l \in T_j} +\ffrac{L}{n_{val}K}\sum_{j=1}^{K}\un{l \in V_j}\\
	(\text{By Assumption \ref{assum:mask-property}} )  &\leq \ffrac{4\beta_{n_{T}} n_{T}}{n}+\ffrac{L}{n}.
	\end{align*}
	Using Mcdiarmid's inequality ( Proposition \ref{prop:Mcdiarmids-ineq}) gives
	\begin{equation*}
	\PP(\DevCV \geq t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}.
	\end{equation*}
	Symmetrically, one has,
	\begin{equation*}
		\PP(\DevCV \leq -t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}.
	\end{equation*}
	Thus,
	$$ \PP(\abs{\DevCV} \geq t) \leq 2\exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}, $$
	which is the desired result. 
\end{proof}


We can mimic some steps in the proof of Lemma \ref{lemma:Dev-CV-UB} to derive a probability upper bound for the term $\DevT$ (cf. Eq \ref{def:dev_train}),


\begin{lemma}\label{lemma:Dev-train-UB}
	Suppose that Assumption~\ref{assum:stability-setting} holds. Then, for all CV schemes verifying Assumption \ref{assum:mask-property},  we have
	\begin{equation*}
		\PP(\abs{\DevT-2\beta_{n_{T}}} \geq t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)},
	\end{equation*}
	where  $L$ is the upper bound of the cost function defined in Assumption~\ref{assum:stability-setting}.
\end{lemma}


	\begin{proof}
Though the proof bears resemblance with the one of Lemma \ref{lemma:Dev-CV-UB}, enough details are given to read it independently. We use McDiarmid's inequality with 
\begin{align*}
f(\mathcal D) &= \ffrac{1}{K}\sum_{j=1}^{K} \left( \ER\left[\alg(T_j),T_j\right] - \risk\big[\alg(T_j)\big]\right) \\
f(\mathcal D^l)  &= \ffrac{1}{K}\sum_{j=1}^{K}  \left( \ER\left[\alg(T_{j,l}),T_{j,l}\right] - \risk\big[\alg(T_{j,l} )\big]\right)
\end{align*}
Since for $l\notin T_j $, $T_j = T_{j,l}$, we find that
\begin{align*}
	\abs{\Delta_l(\DD,O')}	& \leq   \frac{1}{Kn_{T}}  \ \sum_{j=1}^K \indic{l \in T_j}  \left( \ER\left[\alg(T_j),T_j\right] -  \ER\left[\alg(T_{j,l} ),T_{j,l} \right]   + 
	\risk\big[\alg(T_{j,l} )\big] - \risk\big[\alg(T_j)\big] \right)\\
	& \leq   \frac{1}{Kn_{T}}  \ \sum_{j=1}^K \indic{l \in T_j}  \sum_{i \in T_j}\abs{   h (\alg (T_j),O_i) - h(\alg (T_{j,l} ), O_i^l)  } 
	\end{align*}
	with $ h(\alg(T), o  ) = \loss(\alg (T), o) - \EE_{O}\big[\loss(\alg(T),O) \mid \DD_{T } \big] $ and $   (O_i^l)_{i=1,\ldots, n }$ is the same as $(O_i)_{i=1,\ldots, n }$ except the $l$-th element, $O_l$, which is replaced by $O'$. Whenever $ l \in T_j$, it holds that 
	\begin{align*}
	 &| h (\alg (T_j),O_i) - h(\alg (T_{j,l} ), O_i^l) |  \\
	 &=  |\loss (\alg (T_j),O_i) - \loss (\alg (T_{j,l} ), O_i) | \indic {i\neq l} +|\loss (\alg (T_j),O_l) - \loss (\alg (T_{j,l} ), O') | \indic {i =  l} \\
	&\qquad \qquad\qquad \qquad    +   \EE\big[ | \loss(\alg(T_j),O) -\loss(\alg(T_{j,l}),O)  | \mid \DD_{T }, O' \big] \\
	&\leq   2\beta _{n_T}  + L\indic {i =  l} + 2\beta _{n_T} .
	\end{align*}
%To bound the term $\Delta$ corresponding to the maximum deviation of  $\DevT$  we will use the following fact, if $l\in T_j$ then
%		 \begin{equation}
%		 \begin{cases}
%		 		\big \lvert \loss\big(\alg(T_j),O_l\big)-\loss\big(\alg(T_{j,l}),O'\big) \big\rvert \leq L\\
%		 	\big \lvert \loss\big(\alg(T_j),O_j\big)-\loss\big(\alg(T_{j,l}),O_j\big) \big\rvert \leq 2\beta_{n_{T}}\: \text{for} \:j\neq l,
%		 \end{cases}
%		 \end{equation}
%		 and if $l\notin T_j$, one has, 
%		 $$\forall O_j \in T_j\:,\:\loss\big(\alg(T_j),O_j\big)=\loss\big(\alg(T_{j,l}),O_j\big).$$
		 Thus by using 
%		 the same steps as in the previous proof combined with 
		 the identity $\ffrac{1}{K}\sum_{j=1}^{K}  {\indic{l \in T_j} }=\ffrac{n_{T}}{n}$ we get
		 \[\Delta_l(\DD,O')  \leq \ffrac{4\beta_{n_{T}} n_{T}}{n}+\ffrac{L}{n}. \]
		 To derive an upper bound for $\EE[\DevT]$, we use the fact that all the training sets have the same length so that
		$$\EE(\DevT) =\EE\left[\risk\left[\alg(T_1)\right]-\ER\left[\alg(T_1),T_1\right]\right]. $$
		Then, we borrow lemma 7 from \cite{bousquet2002stability} :
		\begin{equation}\label{ineq:stability-expectation-UB}
		\forall T\subset [n] \quad , \quad	\EE\left[\risk\left[\alg(T)\right]-\ER\left[\alg(T),T\right]\right]= \EE\left[\loss\left(\alg(T),O'\right)-\loss\left(\alg(T^l),O'\right)\right].
		\end{equation}
		Where  $\alg(T^{l})$ is the learning rule $\alg$ trained on the sample $\DD_{T}\setminus \{O_l\}\cup \{O'\}$.
		Replacing the left side term by $\EE[\DevT]$ and using Fact \ref{fact:uniform-stab-link} gives
		\begin{equation}
		\abs{\EE[\DevT]} \leq 2\beta_{n_{T}}.
		\end{equation}
		Thus by Mcdiarmid's (Proposition \ref{prop:Mcdiarmids-ineq}), we obtain
		\begin{equation*}
			\PP(Z-2\beta_{n_{T}} \geq t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}.
		\end{equation*}
		Symmetrically, one has
		\begin{equation*}
			\PP(Z-2\beta_{n_{T}} \leq -t) \leq \exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)}
		\end{equation*}
	Thus
		\begin{equation*}
		\PP(\abs{Z-2\beta_{n_{T}}} \geq t) \leq 2\exp{\left(\ffrac{-2nt^2}{(4\beta_{n_{T}}n_{T}+L)^2} \right)},
	\end{equation*}
		and the proof is complete .
	\end{proof}
\begin{remark}\label{remark:bousquet-UB-gen}
	Applying Lemma \ref{lemma:Dev-train-UB} with $T=[n]$ and $K=1$ gives the following probability upper bound
		$$\PP\left(\big|\ER\big[\alg([n]),[n]\big]-\risk\big[\alg([n])\big]-2\beta_n\big| \geq t\right) \leq 2\exp{\left(\ffrac{-2nt^2}{(L+4\beta_{n}n)^2} \right)}.$$
	Thus we retrieve the bound of Theorem 12 in \cite{bousquet2002stability}. It turns out that Lemma \ref{lemma:Dev-train-UB} can be seen as an extension of the latter Theorem to a wide class of CV estimates.
\end{remark}


==> introduction-temp.tex <==
Introduced in \cite{stone74},  cross-validation (\CV) is a most popular tool in statistics for estimating the generalization risk of a learning algorithm. It is also the mainstream approach for model and  parameter selection. Despite its widespread use, it has been shown in several contexts that \CV schemes fail to select the correct model unless the test fraction is negligible in front of the sample size. Unfortunately this excludes the widely used  \Kfold\:\CV. This suboptimality for model selection has been pinned in the linear regression framework by \cite{shao93,shao97,Yuhong2007}, then in other  specific frameworks such as  density estimation (\cite{arlot2008}) and classification (\cite{yang2006}). % However to the best of our knowledge, existing theoretical results regarding   \CV procedures are valid in \emph{restrictive} frameworks, that is  for specific classes of learning algorithms. In fact,
The theoretical properties of \CV\ procedures for model selection in wider settings are
 notoriously difficult to establish. One reason for this is the correlation between the rules learned on each fold.\\

Contrarily to the references cited above  our main focus -to the exception of Section~\ref{sec:model-selec}) is risk estimation, \ie\ we investigate the error made by he \CV\ estimator when estimating the generalization risk of a given learning algorithm. Since this problem is in principle easier than model selection, our negative result  regarding the standard \Kfold\ \CV\ (a lower bound on the \Kfold\ error, as detailed below) has a somewhat more general scope  than existing negative results.  In addition contrarily to most existing works our positive results (upper bounds)  concern the class of \emph{stable} learning algorithms. %, namely \emph{stable algorithms}. % \CV\ procedures in the general framework of stable algorithms.
Indeed our working assumption of  \emph{uniform stability}  encompasses many algorithms such as  Support Vector Machines and Least square regression (\cite{bousquet2002stability}), Stochastic Gradient Descent (\cite{hardt16}) and   neural networks with a simple architecture (\cite{charles18a}). 
 

% Since its introduction in \cite{stone74}, t
The notion of \emph{algorithmic stability} and its consequences in learning theory has received much attention since its introduction in \cite{DEvroy-79}. This property permits to obtain generalization bounds for a large class of a learning algorithms such as  k-nearest-neighbors (\cite{DEvroy-79}), empirical risk minimizers (\cite{kearns1999algorithmic}), regularization networks (\cite{BousquetElisseeff-2000}), bagging (\cite{elisseeff05a}) to name but a few. For an exhaustive review of the different notions of \emph{stability} and their consequences on the generalization risk of a learning algorithms the reader is referred to \cite{kutin2002}.


\paragraph{\bf Related work} 
In \cite{kumar2013near}, \Kfold\:\CV is envisioned under stability assumptions. It is shown that the \Kfold\: risk estimate has a much smaller variance than the simple hold-out estimate and the amount of variance reduction is quantified.  However, the latter results do not imply a universal upper bound regarding  the \Kfold\:neither for risk estimation nor for model selection. Another related work is \cite{celisse2016stability}, who build upon another variant of algorithmic stability, namely $L^q$-\emph{stability} to derive generalization bounds for \emph{leave-p-out} (\lpo) estimates.   Other results regarding \lpo consistency for stable algorithms can be found in \cite{cornec17}.

In contrast with the \lpo case, 
to our best knowledge the literature on algorithmic stability is silent about the consistency of  \Kfold\:CV\,-- the most widely used \CV\ scheme -- in a generic stability setting. Filling this gap is the main purpose of the present paper.


% \subsection{Main contribution}
\paragraph{\bf Contributions and outline}
We introduce the necessary background and notations about \CV\ risk estimation and algorithmic stability in Section~\ref{sec:backround}. \ag{Our main  contributions are gathered in sections ~\ref{sec:CV-UB} ~\ref{sec:KF-LB},~\ref{sec:BKF-UB},~\ref{sec:model-selec} and  may be summarized as follows:
\begin{enumerate}
	\item We state and prove a generic upper bound for the generalization gap (Section \ref{sec:CV-UB}) (estimation error) of a wide class of \CV procedures. Our result can be seen as an extension of the previous work of \cite{bousquet2002stability} who studied only the usual training error and the \loo estimate (which is not used in practice). However,  the "generic upper bound" obtained isn't efficient unless the test fraction is negligible in front on the sample size. which excludes the \Kfold and the repeated \Kfold. 
	\item Due to this negative result , one may wonder if we can guarantee that \Kfold \:\CV
\end{enumerate}
}
Section~\ref{sec:CV-UB} is intended to give some context about existing guarantees regarding a wide class of \CV\ schemes, namely those satisfying a balance condition, Assumption~\ref{assum:mask-property} below. We  state and prove a generic upper bound on the error of the generalization risk estimate for stable algorithms generalizing comparable results from \cite{celisse2016stability,cornec17}. This upper bound is satisfactory for the \lpo\ scheme in the sense that it yields in this case the usual rate of  a PAC generalization  bound converging to zero with the sample size at rate $\mathcal{O}\left(\sqrt{\ffrac{1}{n}}\right)$, making it a \emph{sanity-check bound} (\cite{kearns1999algorithmic}). However, for the  \Kfold\:CV, the obtained upper bound is not satisfactory, in so far as  it does not vanish as $n\rightarrow \infty$. 

% Although the results in \cite{celisse2016stability,cornec17} are valid under weaker assumptions than ours, we start off with deriving
% a generic  upper bound in Section~\ref{sec:CV-UB} which holds under uniform stability
% (Theorem~\ref{theo:CV-stable-bound}) with a different technique of proof, which yields a control of the \lpo error  (Corollary~\ref{cor:lpo-UB}). Such a control of the  error is limited to the  \emph{leave-one-out} (\emph{loo}) in the literature so that we state and the result in the general case for the sake of completeness. 
%we add, for the sake of completeness, the results regarding \lpo\, since our techniques proofs are very different from those in the latter works.
%However, the latter procedure can be computationally heavy and it is rarely used in practice \as{phrase à améliorer en fonction du positionnement juste au dessus}.
%We generalize an upper bound on the \CV error (Section~\ref{sec:CV-UB}) which was limited to \emph{leave-one-out} (\emph{loo}) in the existing literature.
% This upper bound is satisfactory for the \lpo\, scheme in the sense that it yields in this case the usual rate of  a PAC generalization  bound converging to zero with the sample size at rate $\mathcal{O}\left(\sqrt{\ffrac{1}{n}}\right)$, making it a \emph{sanity-check bound} (\cite{kearns1999algorithmic}). However, for the  \Kfold\:CV, the obtained upper bound is not satisfactory, in so far as  it does not vanish as $n\rightarrow \infty$. 

Our main  contributions are gathered in sections~\ref{sec:KF-LB},~\ref{sec:BKF-UB},~\ref{sec:model-selec} and  may be summarized as follows:
\begin{enumerate}%[$\bullet$] 
\item One may wonder whether the looseness of the bound for the specific case of the \Kfold\  is just an artifact from our proof. % , which is based on existing  arguments from the \CV\ literature \ag{?}.
  We answer in the negative by deriving a lower bound for the \Kfold\:(Section~\ref{sec:KF-LB}). The latter bound shows that under the uniform stability assumption alone,  one cannot construct a vanishing universal upper bound  for the \Kfold\ estimation error for fixed $K$ \ag{?}. % can be inconsistent. 
  	\item In view of the latter negative result we propose a general debiased version of the \Kfold\: following in the footsteps of \cite{BURMAN89,arlot2016VFchoice} who considered only the frameworks of linear regression and density estimation. Our procedure encompasses any uniformly stable learner. For this debiased \Kfold\:scheme, we derive (Section \ref{sec:BKF-UB}) a PAC generalization bound of order $\mathcal{O}\left(\sqrt{\ffrac{1}{n}}\right)$. As an example of application, we show that the debiased \Kfold\:permits to select a model within a finite collection in a  risk consistent manner (Section \ref{sec:model-selec}), in other words, the excess risk of the selected model tends to $0$ as $n\rightarrow \infty$. Finally we demonstrate empirically (Section~\ref{sec:experiments}) the added value of the debiased \Kfold\:compared with the standard one in terms of the test error of the selected model.
        \end{enumerate}
We do not claim originality regarding Section~\ref{sec:CV-UB} which is merely intended to provide  some context about the lack of guarantee regarding the standard \Kfold\  in a self-contained manner and to motivate the rest of this work.  % lower bound (Section~\ref{sec:KF-LB}) and the debiased \Kfold\ (Section~\ref{sec:BKF-UB}). 
                 The novelty of this paper  mainly resides in Contribution 1 (lower bound for the \Kfold) and Contribution 2 (debiased version) listed above. Indeed we believe that the generic lower bound and the debiased scheme that we promote are the first of their kind for the \Kfold\ in a general stability framework. 
        
% Therefore, we wanted to study the \Kfold\: for stable learners, and we believe that we've found a way to ensure the consistency of this procedure.
 

%%% Local Variables:
%%% TeX-master: "main_crossval.tex"
%%% End:


==> introduction_bak.tex <==
Introduced in \cite{stone74},  cross-validation (\CV) is a most popular tool in statistics for estimating the generalization risk of a learning algorithm. It is also the mainstream approach for model and  parameter selection. Despite its widespread use, it has been shown in several contexts that \CV schemes fails to select the correct model unless the test fraction is negligible in front of the sample size. Unfortunately this excludes the widely used  \Kfold\:\CV. This lack of consistency has been pinned in the linear regression framework by \cite{shao93,shao97,Yuhong2007}, then in other frameworks such as  density estimation (\cite{arlot2008}) and classification (\cite{yang2006}). However to the best of our knowledge, existing results regarding  theoretical consistency of \CV procedures are valid in \emph{restrictive} frameworks, that is  for specific classes of learning algorithms. In fact, the theoretical properties of \CV estimates in wider settings are
notoriously difficult to establish due to the correlation between the rules learned on each fold.\\
In constrast the present paper studies \CV procedures in the general framework of stable algorithms. Our working assumption of  \emph{uniform stability}  encompasses many algorithms such as  Support Vector Machines and Least square regression (\cite{bousquet2002stability}), Stochatic Gradient Descent (\cite{hardt16}) and   neural networks with a simple architecture (\cite{charles18a}).

% Since its introduction in \cite{stone74}, t
The notion of \emph{algorithmic stability} and its consequences in learning theory has received much attention since its introduction in \cite{DEvroy-79} . Indeed, this notion permits to obtain generalization bounds for a large class of a learning algorithms such as  K-nearest-neighbors (\cite{DEvroy-79}) , empirical risk minimizers (\cite{kearns1999algorithmic}), regularization networks (\cite{BousquetElisseeff-2000}), Bagging (\cite{elisseeff05a}) to name but a few. For an exhaustive review of the different notions of \emph{stability} and their consequences on the generalization risk of a learning algorithms the reader is reffered to \cite{kutin2002}.

% \subsection{Main contribution}
%\paragraph{\bf Contributions}
Our contributions may be summarized as follows:
\begin{itemize}[$\bullet$] 
	\item We generalize an upper bound on the \CV error (Section~\ref{sec:CV-UB}) which was limited to \emph{leave-one-out} (\emph{loo}) in the existing litterature. This upper bound is satisfactory for the \emph{leave-p-out} (\emph{lpo}) scheme in the sense that it enjoys the usual rate of  a PAC generalization  bound $\mathcal{O}\left(\sqrt{\ffrac{1}{n}}\right)$, making it a \emph{sanity-check bound} (\cite{kearns1999algorithmic}). However, for the  \Kfold\:CV, the obtained upper bound is not consistent, in so far as  it does not vanish as $n\rightarrow \infty$. One may wonder whether this is just an artifact from our proof. We answer in the negative by deriving a lower bound specific to the \Kfold\:(Section \ref{sec:KF-LB}). The latter bound shows that under the uniform stability assumption alone,  \Kfold\:CV can be inconsistent.
	\item In view of the latter inconsistency result we propose a general debiased version of the \Kfold\: following in the footsteps of \cite{BURMAN89,arlot2016VFchoice} who considered only the frameworks of linear regression and density estimation. Our procedure encompasses any uniformly stable learner. For this debiased \Kfold\:scheme, we derive (Section \ref{sec:BKF-UB}) a PAC generalization bound of order $\mathcal{O}\left(\sqrt{\ffrac{1}{n}}\right)$. As an example of application, we show that the debiased \Kfold\:permits to select a model within a finite collection in a  risk consistent manner (Section \ref{sec:model-selec}), in other words, the excess risk of the selected model tends to $0$ as $n\rightarrow \infty$. Finally we demonstrate empirically (Section~\ref{sec:experiments}) the added value of the debiased \Kfold\:compared with the standard one in terms of the test error of the selected model.
        \end{itemize}
       
\subsection{Related work} 
In \cite{kumar2013near}, \Kfold\:\CV\, is envisioned under stability assumptions. It is shown that the \Kfold\: risk estimate has a much smaller variance than the simple hold-out estimate and the amount of variance reduction is quantified.  However, the latter results do not imply consistency of the \Kfold\:neither for risk estimation nor for model selection. Another related work is \cite{celisse2016stability}, who build upon another variant of algorithmic stability, namely $L^q$-\emph{stability} to derive generalization bounds for \emph{lpo} estimates.   Other results regarding \emph{lpo} consistency when working with stable algorithms can be found in \cite{cornec17}. Although the results in \cite{celisse2016stability,cornec17} uses a  type of stability that is weaker than \emph{uniform} stability, we add, for the sake of completeness, the results regarding \emph{lpo} since our techniques proofs are very different from those in the latter works. However, the latter procedure can be computationally heavy and it is rarely used in practice \as{phrase à améliorer en fonction du positionnement juste au dessus}.

To our best knowledge, the literature on algorithmic stability is silent about the consistency of  \Kfold\:CV\,-- the most widely used one -- in a generic stability setting. Filling this gap is the main purpose of the present paper.
% Therefore, we wanted to study the \Kfold\: for stable learners, and we believe that we've found a way to ensure the consistency of this procedure.
 



==> unbiased-cv.tex <==

\begin{lemma}[Arlot]
	If the algorithm $\alg$ verifies :
	\begin{equation}\label{eq:first-stability-def}
	\EE\left[\ER\left[\alg,[n]\right]-\TR\left[\alg\left([n]\right)\right]\right] =\ffrac{C}{n},
	\end{equation}
	for some constant $C\in \rset$ then
	$$\EE\left[ \ER^{corr}_{\mathrm{Kfold}}\right]=\EE\left[\TR\left[\alg\left([n]\right)\right]\right]$$
\end{lemma}

\ag{D'une manière générale on peut démontrer cela :\\
Si $$\EE\left[\ER\left[\alg,[n]\right]-\TR\left[\alg\left([n]\right)\right]\right] =\ffrac{C}{n^a}$$ alors la K-fold pénalisation
  \begin{align}\label{def:pen-Kfold}
\rCV^{\mathrm{pen}}\big[\alg,&V_{1:K}\big] = \ER\left[\alg([n]),[n]\right]\nonumber \\+ &\ffrac{x}{K}\sum_{j=1}^{K}\left[\ER\left[\alg(T_j),V_j\right]-\ER\left[\alg(T_j),T_j)\right]\right] . 
\end{align}
est sans biais pour $x=(K-1/K)^a$}

\ag{Lien avec la stabilité : l'équation 
		$$\EE\left[\ER\left[\alg,[n]\right]-\TR\left[\alg\left([n]\right)\right]\right] =\ffrac{C}{n}$$,
		est équivalente à 
		$$\forall i \in [n] \quad,\quad   \EE\left[\bigg\lvert \loss\left(\alg\left([n]\right),O_i\right) -\loss\left(\alg\left([n]^{i}\right),O_i\right)\bigg\rvert\right]=\mathcal{O}\left(\frac{1}{n_T}\right).$$
}
In the rest of this section we are interested in the regression problem $O=(X,Y) \in \mathcal{X}\times \mathbb{R}$  where 
$$Y=\phi(X)^{\top}\theta^{\star}+\varepsilon$$
for some random noise $\varepsilon$ independent of $X$ with $\EE\left[\varepsilon\right]=0$ and $\EE\left[\varepsilon^2\right]=\sigma^2$.\\
\subsection{Ordinary least square}
First, let $\Phi\in\rset^{n\times d}$ denote the input matrix, $y=\left(Y_1,Y_2,\dots,Y_n\right)$ the response vector and $\lVert \alpha\rVert_{2}^2=\sum_{i=1}^{n}\alpha_i^2 $ is the $\loss$-2 norm of $\alpha$. Now, we start by showing that ordinary least squares  verifies Equation \ref{eq:first-stability-def}.

\begin{theorem}
	The ordinary least square algorithm 	$\alg\left(\DD_n,X\right)=\phi\left(X\right)\hat\theta$  with 
	\begin{equation}\label{eq:OLS-def}
	\hat \theta =\argmin_{\theta\in \mathbb{R}^d}\ffrac{1}{n}\lVert y-\Phi\theta\rVert_{2}^2,
	\end{equation} 
	
	satisfies Equation \ref{eq:first-stability-def} furthermore $\alg$ is $\mathcal{O}\left(1/n\right)$ \emph{point wise hypothesis stable} \ie
	
	$$ \forall i \in T \quad,\quad   \EE\left[\bigg\lvert \loss\left(\alg\left(T\right),O_i\right) -\loss\left(\alg\left(T^{\backslash i}\right),O_i\right)\bigg\rvert\right]=\mathcal{O}\left(\frac{1}{n_T}\right).  $$
\end{theorem}
\subsection{Ridge regression}
	The ordinary least square algorithm 	$\alg\left(\DD_n,X\right)=\phi\left(X\right)\hat\theta$  with 
\begin{equation}\label{eq:ridge-def}
\hat \theta =\argmin_{\theta\in \mathbb{R}^d}\ffrac{1}{n}\lVert y-\Phi\theta\rVert_{2}^2+\lambda\lVert\theta\rVert_{2}^2,
\end{equation} 

satisfies,
$$\EE\left[\ER\left[\alg,[n]\right]-\TR\left[\alg\left([n]\right)\right]\right]=A_1+\frac{\sigma^2 A_2}{n},$$

where 
$$ A_1=\lambda^2\EE\left[ \theta_*^{\top}(\widehat{\Sigma}+\lambda I)^{-2} \left(\widehat{\Sigma}-\Sigma\right) \theta_*\right]$$
$$ A_2=  \EE\left[\operatorname{tr}\left[\left(\widehat{\Sigma}-\Sigma\right)\widehat{\Sigma}(\widehat{\Sigma}+\lambda I)^{-2}\right]\right]+\EE\left[\operatorname{tr}\left(\widehat{\Sigma}(\widehat{\Sigma}+\lambda I)^{-1}\right)\right] $$
